EPspectra: A Formal Toolkit for Developing DSP Software Applications

The software approach to developing Digital Signal Processing (DSP) applications brings some great features such as flexibility, re-usability of resources and easy upgrading of applications. However, it requires long and tedious tests and verification phases because of the increasing complexity of the software. This implies the need of a software programming environment capable of putting together DSP modules and providing facilities to debug, verify and validate the code. The objective of the work is to provide such facilities as simulation and verification for developing DSP software applications. This led us to develop an extension toolkit, Epspectra, built upon Pspectra, one of the first toolkits available to design basic software radio applications on standard PC workstations. In this paper, we first present Epspectra, an Esterel-based extension of Pspectra that makes the design and implementation of portable DSP applications easier. It allows drastic reduction of testing and verification time while requiring relatively little expertise in formal verification methods. Second, we demonstrate the use of Epspectra, taking as an example the radio interface part of a GSM base station. We also present the verification procedures for the three safety properties of the implementation programs which have complex control-paths. These have to obey strict scheduling rules. In addition, Epspectra achieves the verification of the targeted application since the same model is used for the executable code generation and for the formal verification.

==> kim05epspectra <==
@phdthesis{bose:99,
   author={Vanu G. Bose},
   title={Design and Implementation of Software Radios Using a General Purpose Processor},
   school={MIT},
   month={June},
   year=1999
}
@mastersthesis{brett:00,
   author={Brett W. Vasconcellos},
   title={Parallel Signal-Processing for Everyone},
   school={MIT},
   month={Feb},
   year=2000
}

@misc{sco:web,
  title={Overview of the Global System for Mobile Communications},
  author={John Scourias},
  howpublished={http://ccnga.uwaterloo.ca/~jscouria/GSM/gsmreport.html}
}
@misc{gsm:web,
  title ={An overview of the GSM system},
  author={GSM Association},
  howpublished={http://www.gsm.org}
}


@Book{mouly:93,
   author={Michel Mouly and Marie B. Pautet},
   title={The GSM System for Mobile Communications},
   publisher={Europe Media Duplication S.A},
   series={ISBN 2-9507190-07},
   year=1993
}

@electronic{berry:99:primer,
  author={G\'{e}rard Berry},
  title={The Esterel v5 Language Primer},
  url={http://www.esterel.org},
  year=1999
}

@inproceedings{berry:89,
    author={G\'{e}rard Berry},
    title={Real time programming: Special purpose or general purpose languages},
    booktitle={{IFIP World Computer Congress},
    publisher={Elsevier Science},
    pages={11-17},
    year=1989
}
@inproceedings{berry:96,
    author ={G\'{e}rard Berry},
    title ={Constructive Semantics of Esterel: From Theory to Practice (Abstract)},
    booktitle ={Algebraic Methodology and Software Technology},
    pages ={225},
    year=1996,
    url={citeseer.ist.psu.edu/article/berry96constructive.html}


@inproceedings{berry:93,
    author ={G\'{e}rard Berry},
    title ={Preemption in Concurrent Systems},
    booktitle ={Foundations of Software Technology and Theoretical Computer Science},
    pages={72-93},
    year=1993
}

@inproceedings{jagadeesan95safety,
    author={L. J. Jagadeesan and C. Puchol and J. E. Von Olnhausen},
    title={Safety Property verification of Esterel programs and applications to telecommunications software},
    booktitle={the 7th International Conference On Computer Aided Verification},
    volume={939},
    publisher={Springer Verlag},
    pages={127-140},
    year=1995
}

@incollection{94:european,
  title={European digital cellular telecommunication system},
  booktitle={ETS 300 580-2, Version 6.10.},
  publisher={ETSI},
  month={Sep.},
  year=1994
}

@article{murota:81:gmsk,
  title={GMSK Modulation for Digital Radio Telephony},
  author={K. Murota and K. Hirade},
  journal ={IEEE Trans. on Communications},
  volume ={com-29},
  number ={7},
  pages ={1044-1050},
  year =1981
}

@inproceedings{bouali:98:xeve,
  author={Amar Bouali},
  title={Xeve: an Esterel Verification Environment},
  booktitle={the 10th International Conference on Computer Aided Verification},
  volume={1427},
  publisher={LNCS},
  year =1998
}

@inproceedings{arditi:99,
  author={Laurent Arditi and Amar Bouali and others},
  title ={Using Esterel and Formal Methods to Increase the Confidence in the Functional Validation of a Commercial DSP},
  booktitle={FLoC'99, 4th ERCIM Workshop of Formal Methods for Industrial Critical Systems},
  year=1999
}

@article{bryant:86,
author ={Randal E. Bryant},
title = {Graph-Based Algorithms for Boolean Function Manipulation},
journal = {IEEE Transactions on Computer},
volume = {C-35},
number = {8},
month = {Aug.},
year =1986,
pages = {677-691}
}

@manual{berry:99:xes,
author ={G\'{e}rard Berry and Esterel team},
title ={The Esterel v5.92 System Manual},
address ={http://www.esterel.org},
year =1999
}

@inproceedings{ simone:93,
  author = {R. de Simone and A. Ressouche},
  title = {Compositional semantics of Esterel and Verification by Compositional Reductions},
  booktitle={the 5th International Conference on Computer Aided Verification},
  publisher={LNCS},
  pages ={818},
  year =1994
}

@inproceedings{ sentovitch:96,
  author = {Ellen M. Sentovitch and Horia Toma and Gerard Berry},
  title = {Latch Optimization in Circuits Generated from High-Level Descriptions},
  booktitle={the 8th International Conference on Computer Aided Verification},
  publisher={IEEE},
  year =1996
}

@techreport{ brayton:92:sis,
    author ={Ellen M. Sentovich and Kanwar Jit Singh and Luciano Lavagno and Cho Moon and Rajeev Murgai and Alexander Saldanha and Hamid Savoj and Paul R. Stephan and Robert K. Brayton and others},
    title ={SIS: A system for sequential circuit synthesis},
    institution ={Univ. of California Berkeley},
    number={UCB/ERL M92/41},
    year =1992
}

@inproceedings{closse:03,
  author ={Etienne Closse and Michel Poize and Jacques Pulou and Joseph Sifakis and Patrick Venter and Daniel Weil and Sergio Yovine},
  title ={TAXYS: a Tool for Developing and Verifying Real-Time Properties of Embedded Systems},
  booktitle={the 13th International Conference on Computer Aided Verification},
  publisher={Springer-Verlag Heidelberg},
  volume={2102},
  month={Jun.},
  year =2003
}

@article{ johnsson:84,
    author ={Thomas Johnsson},
    title = {Efficient Compilation of Lazy Evaluation},
    journal ={SIGPLAN Notices},
    volume ={39},
    issue={4},
    publisher ={ACM Press},
    pages ={125-138},
    month={Apr.},
    year =2004
}

@article{ jensen94,
  author ={E. Douglas Jensen},
  title ={Eliminating the Hard/Soft Real-Time Dichotomy},
  journal={Computing and Control Engineering},
  publisher={Digital Equipment Corp.},
  volume={8},
  issue={1},
  pages={15-19},
  month={Feb.},
  year =1997
}

@incollection{ jagannathan:95,
  author ={R. Jagannathan},
  title ={Dataflow models},
  publisher ={Parallel and Distributed Computing Handbook. McGraw-Hill},
  year =1996
}
@inproceedings{jones:01,
  author={Michael B. Jones and Stefan Saroin},
  title={Predictability Requirements of a Soft Modem},
  booktitle={ACM SIGMETRICS Conference on Measurement and Modeling of Computer Systems},
  address={Cambridge USA},
  month={June},
  year=2001
}

@article{allan95sofwarepipeling,
    author ={Vicki H. Allan and Reese B. Jones and Randall M. Lee and Stephen J. Allan},
    title ={Software pipeling},
    booktitle ={ACM Computing Surveys},
    journal ={SIGPLAN Notices},
    volume ={27},
    number ={3},
    month={Sep.},
    publisher ={ACM Press},
    pages ={367-432},
    year =1995
}

@article{hal:91:lustre,
   author={N. Halbwachs and P. Caspi and P. Raymond and D. Pilaud},
   title={The synchronous dataflow programming language Lustre},
   journal={IEEE},
   volume={79},
   number={9},
   pages={1305-1320},
   month={Sep.},
   year=1991
   }

@article{hal:92,
   author ={N. Halbwachs and F. Lagnier and C. Ratel},
   title ={Programming and verifying real-time systems by means of the synchronous data-flow programming language Lustre},
   journal ={IEEE Transactions on Software Engineering, Special Issue on the Specification and Analysis of Real-Time Systems},
   publisher={IEEE},
   month={Sep.},
   year=1992
   }

@article{hal:97,
   author={N. Halbwachs and Y.E. Proy and P. Roumanoff},
   title={Verification of real-time systems using linear relation analysis},
   journal={Formal Methods in System Design},
   volume={11},
   number={2},
   pages={157-185},
   publisher={Kluwer},
   month={Aug.},
   year={1997}
}

@inproceedings{hal:93,
   author={N. Halbwachs and F. Lagnier and P. Raymond},
   title={Synchronous observers and the verification of reactive systems},
   booktitle={3rd Int. Conf. on Algebraic Methodology and Software Technology (AMAST)'93},
   month={Jun.},
   publisher={Springer Verlag},
   year=1993
   }


@inproceedings{bcdp99,
    author ={S. Bensalem and P. Caspi and C. Parent-Vigouroux and C. Dumas},
    title ={A Methodology for Proving Control Systems with {Lustre} and {PVS}},
    booktitle ={7th Working Conference on Dependable Computing for Critical Applications},
    volume ={12},
    publisher ={IEEE},
    pages ={89-107},
    month={Jan.},
    year =1999
}

@inproceedings{jeannet:99,
    author ={B. Jeannet and N. Halbwachs and P. Raymond},
    title={Dynamic Partitioning in Analyses of Numerical Properties},
    booktitle={Static Analysis Symposium (SAS)'99},
    month ={Sep.},
    year=1999
}

@inproceedings{hal:99,
    author ={N. Halbwachs and P. Raymond},
    title ={Validation of Synchronous Reactive Systems: from Formal Verification to Automatic Testing},
    booktitle={Asian Computing Science Conference},
    publisher={LNCS 1742, Springer Verlag},
    month ={Dec.},
    year =1999
}

@inproceedings{raymond:98,
    author ={P. Raymond and D. Weber and X. Nicollin and N. Halbwachs},
    title={Automatic Testing of Reactive Systems},
    booktitle={19th IEEE Real-Time Systems Symposium},
    month={Dec.},
    year =1998
}

@article{ben:91:signal,
    author={Albert Benveniste and Paul Le Guernic and Christian Jacquemot},
    title={Synchronous programming with events and relations: the SIGNAL language and its semantics},
    journal={Science of Computer Programming},
    publisher={Elsevier},
    volume={16},
    issue={2},
    pages={103-149},
    month={Sep.},
    year=1991
}

@article{harel:87,
    author={David Harel},
    title={Statecharts: a visual formalism for complex systems},
    journal={Science of Computer Programming},
    publisher={Elsevier},
    volume={8},
    issue={3},
    pages={231-274},
    month={Jun.},
    year=1987
}

@inproceedings{borgne:96,
  author={Michel Le Borgne and Hervé Marchand and Éric Rutten and Mazen Samaan},
  title={Formal Verification of SIGNAL Programs: Application to a Power Transformer Station Controller},
  booktitle={5th International Conf. on Algebraic Methodology and Software Technology (AMAST)'96},
  publisher={LNCS Springer},
  volume={1101},
  pages={271-285},
  month={Jul.},
  year=1996
}

@inproceedings{burch:90,
    author={J. R. Burch and E. M. Clarke and K. K. McMillan and D. L. Dill and J. Hwang},
    title={Symbolic model checking: $10^{20}$ states and beyond},
  booktitle ={IEEE Symposium on Logic in Computer Science},
  publisher ={IEEE},
  pages={428-439},
  month={Jun.},
  year=1990
}

@techreport{guernic:91,
  author={Paul Le Guernic and Michel Le Borgne and  Thierry Gautier andClaude Le Maire},
  title={Programming Real-Time Applications with SIGNAL},
  institution={IRISA},
  address={35042 Rennes},
  number={RR 1446},
  month={June},
  year=1991
}

@techreport{alpern:84,
  author ={Bowen Alpern and Fred B. Schneider},
  title={Defining Liveness},
  institution={Cornell University},
  address={Ithaca NY 14853},
  number={TR 85-650},
  month={Oct.},
  year=1984
}

@techreport{alpern:85,
  author ={Bowen Alpern and Alan J. Demers and Fred B. Schneider},
  title={Safety without Stuttering},
  institution={Cornell University},
  address={Ithaca NY 14853},
  number={TR 85-708},
  month={Oct.},
  year=1985
}

@article{clarke:86,
  author={E. M. Clarke and E. A. Emerson and K. L. McMillan},
  title={Automatic verification of finite-state concurrent systems using temporal logic specifications},
  journal={ACM Transactions on Programming Languages and Systems},
  publisher={ACM Press},
  volume={8},
  issue={2},
  pages={244-263},
  month={Apr.},
  year=1986
}

